Observation of $D \to a_{0}(980)\pi$ in the decays $D^{0} \rightarrow \pi^{+}\pi^{-}\eta$ and $D^{+} \rightarrow \pi^{+}\pi^{0}\eta$

We report the first amplitude analysis of the decays $D^{0} \to \pi^{+} \pi^{-} \eta$ and $D^{+} \rightarrow \pi^{+}\pi^{0}\eta$ using a data sample taken with the BESIII detector at the center-of-mass energy of 3.773 GeV, corresponding to an integrated luminosity of 7.9 ${\rm fb}^{-1}$. The contribution from the process $D^{0(+)} \to a_{0}(980)^{+} \pi^{-(0)}$ is significantly larger than the $D^{0(+)} \to a_{0}(980)^{-(0)} \pi^{+}$ contribution. The ratios $\mathcal{B}(D^{0} \rightarrow a_{0}(980)^{+}\pi^{-})/\mathcal{B}(D^{0} \rightarrow a_{0}(980)^{-}\pi^{+})$ and $\mathcal{B}(D^{+} \rightarrow a_{0}(980)^{+}\pi^{0})/\mathcal{B}(D^{+} \rightarrow a_{0}(980)^{0}\pi^{+})$ are measured to be $7.5^{+2.5}_{-0.8\,\mathrm{stat.}}\pm1.7_{\mathrm{syst.}}$ and $2.6\pm0.6_{\mathrm{stat.}}\pm0.3_{\mathrm{syst.}}$, respectively. The measured $D^{0}$ ratio disagrees with the theoretical predictions by orders of magnitudes, thus implying a substantial contribution from final-state interactions.

==> introduction.tex <==
Recently, the observation of exotic state candidates consisting of at least one heavy quarks raises amount of theoretical interpretations and related experimental measurements. 
For the hadrons consisting of only $u$, $d$ and $s$ quarks, the scalar mesons are the candidates for exotic states, 
e.g. the $f_{0}(980)$, considered as a $K\bar{K}$ molecule state, 
so that its partner particle $a_{0}(980)$ whose iso-spin is one is also considered as a exotic state candidate~\cite{Guo:2017jvc}, which 
is strongly supported by the observation of $D_{s}^{+} \rightarrow a_{0}(980)^{+/0}\pi^{0/+}$~\cite{BESIII:2019jjr}. 
However, theoretical interpretations still can not conclude the $a_{0}(980)$ 
is a $K\bar{K}$ molecule or the other unconventional state~\cite{Molina:2019udw,Hsiao:2019ait,Ling:2021qzl}. 

More experimental measurements for $D_{s}^{+}$ decays have been performed these years, among them, the observation of 
$D_{s}^{+} \to a_{0}(980)^{+} \rho^{0}$~\cite{BESIII:2021aza} indicates that the $a_{0}(980)$ generated through the triangle singularity in $D_{s}$ decays ~\cite{Yu:2021euw}; 
the observation of $D_{s}^{+} \to a_{0}(1817)^{+/0} \pi^{0/+}$~\cite{BESIII:2021anf,BESIII:2022wkv} 
strongly supports the $K^{*}\bar{K}^{*}$ molecule model for $a_{0}(1817)$~\cite{Wang:2021jub,Guo:2022xqu}.
Since $a_{0}(1817)$ is expected as an excited state of $a_{0}(980)$ and its $K^{*}\bar{K}^{*}$ molecule model 
is similar with the $K\bar{K}$ molecule model for $a_{0}(980)$. Therefore, this observation also support the $K\bar{K}$ molecule explanation for $a_{0}(980)$.

%Here, $a_{0}(1817)$ was firstly explained as $a_{0}(1710)$, the iso-spin vector partner of $f_{0}(1710)$~\cite{BESIII:2021anf}. Which indicates $f_{0}(1710)$ being $K^{*}\bar{K}^{*}$ molecule and challenges the explanation of $f_{0}(1710)$ being glue ball and the experimental measurement of the upper limit of $f_{0}(1710) \to \eta \eta^{\prime}$~\cite{BESIII:2022iwi}. Therefore, theoretical interpretation~\cite{Guo:2022xqu} points out that $a_{0}(1817)$ should be the iso-spin vector partner of $X(1812)$. 


%~{\footnote {Here, the $a_{0}(1817)$ was firstly explained as the iso-spin vector partner of $f_{0}(1710)$, indicates $f_{0}(1710)$ being $K^{*}\bar{K}^{*}$ molecule, which challenges the explanation of $f_{0}(1710)$ being glue ball and the experimental observation of the upper limit of $f_{0}(1710) \to \eta \eta^{\prime}$ in arXiv.2202.00623.}}

%{\footnote %{However, in arXiv.2202.00623, the upper limit of $f_{0}(1710) \to \eta \eta^{\prime}$ indicates the $f_{0}(1710)$ is a glue ball, which is also disagree with the $K^{*}\bar{K}^{*}$ molecule model.}}, 

%therefore it also indicates the $a_{0}(980)$ as a $K\bar{K}$ molecule.

The above serious experimental studies are for $D_{s}$ decays, there are few experimental measurements for $D^{0}$ and $D^{+}$ decays, 
which have been proposed by theoretical interpretations~\cite{Ikeno:2021kzf,Duan:2020vye}.
Previous experimental studies involving $a_{0}$ intermediate states are all using $K\bar{K}$ channel to reconstruct. Both CLEOc and LHCb observe $D^{0} \to a_{0}(1450)^{\pm}\pi^{\mp}$ in the study of $D^{0} \to K_{S}^{0}K^{\pm}\pi^{\mp}$~\cite{CLEO:2012obf,LHCb:2015lnk}, 
while CLEOc reports only $D^{0} \to a_{0}(1450)^{\pm}\pi^{\mp}$ evidence is found and LHCb reports significant larger contribution from $D^{0} \to a_{0}(980)^{\pm}\pi^{\mp}$ compared with $D^{0} \to a_{0}(1450)^{\pm}\pi^{\mp}$. 
Further more, in the study performed by LHCb, the decay $D^{0} \to a_{0}(980)^{+}\pi^{-}$ is observed, while for $D^{0} \to a_{0}(980)^{-}\pi^{+}$, 
two different amplitude models with and without this decay both give good fit.
So the conclusion on the contribution for the decays $D^{0} \to a_{0}(1450)^{\pm}\pi^{\mp}$ and $D^{0} \to a_{0}(980)^{\pm}\pi^{\mp}$ are not consistent for these two analyses. And for $a_{0}(980)$, the asymmetry between $D^{0} \to a_{0}(980)^{+}\pi^{-}$ and $D^{0} \to a_{0}(980)^{-}\pi^{+}$ is also found according to the LHCb analysis, which is quite different with the equivalent case observed for $D_{s}^{+} \to a_{0}(980)^{+}\pi^{0}$ and $D_{s}^{+} \to a_{0}(980)^{0}\pi^{+}$~\cite{BESIII:2019jjr}.
Here, another search of CP violation in $D^{0} \to \pi^{-}\pi^{+}\eta$ performed by Belle also shows the branching fraction of the decay $D^{0} \to a_{0}(980)^{+}\pi^{-}$ being significantly larger than that of $D^{0} \to a_{0}(980)^{-}\pi^{+}$ according to the given projections on $m(\pi^{+}\eta)$ and $m(\pi^{-}\eta)$~\cite{Belle:2021dfa}. 
To be convenient, we define the ratio $r_{+/-}=\frac{\mathcal{B}(D^{0} \rightarrow a_{0}(980)^{+}\pi^{-})}{\mathcal{B}(D^{0} \rightarrow a_{0}(980)^{-}\pi^{+})}$.

In theory, a interpretation predicts the branching ratios of $D^{0} \rightarrow a_{0}(980)^{+}\pi^{-}~(a_{0}(980)^{-}\pi^{+})$ (here $a_{0}(980)^{\pm} \to K_{S}^{0}K^{\pm}$) being $1.3 \times 10^{-5}$ ($2.9\times 10^{-4}$) based on topological amplitude with assuming $a_{0}(980)$ being two-quark states or four-quark states~\cite{Cheng:2022vbw}. 
%The predicted branching fraction of $D^{0} \rightarrow a_{0}(980)^{+}\pi^{-}$ is much smaller than the mean values obtained from the studies of $D^{0} \to K_{S}^{0}K^{+}\pi^{-}$, while 
%the result of $D^{0} \rightarrow a_{0}(980)^{-}\pi^{+}$ is comparable with experimental measurement. 
The predicted branching fraction of $a_{0}(980)^{-}$ mode is larger than the one of $a_{0}(980)^{+}$ mode, which is opposite with the mean value of experimental measurement~\cite{CLEO:2012obf,LHCb:2015lnk}. Theory and experiment gives different magnitudes for the ratio between the two decays:
\begin{eqnarray}
\begin{aligned}
r_{+/-,ph}&=4.5\times10^{-2}, \\
r_{+/-,ex}&=4.6\pm5.8,
\end{aligned}
\end{eqnarray}
where the sub-index $ph$ and $ex$ represent the theoretical prediction and experimental measurement.
$r_{ph}$ is smaller than the mean value of $r_{ex}$ by two orders of magnitude, which implies the unknown mechanism for the decays of $D^{0} \to a_{0}(980)^{\pm}\pi^{\mp}$.
However, the uncertainties of the two branching fractions for experimental measurement are so large, which makes the $r_{ex}$ cover 0 within the uncertainty. 
Previous branching fraction measurement for $D^{0} \to \pi^{+} \pi^{-} \eta$ based on 2.93fb$^{-1}$ of $\psi(3770)$ data accumulated by BESIII detector located at the Beijing Electron Position Collider~\cite{Yu:IPAC2016-TUYA01} shows there are about 450 signal candidate~\cite{BESIII:2019xhl}.
Therefore, we perform an amplitude analysis to this decay to verify whether there is the disagreement of magnitude between theoretical interpretation and experimental measurement in $D^{0} \to a_{0}^{\pm} \pi^{\mp}$.

The detail description of the BESIII detector and the upgraded multi-gap resistive plate chambers used in the time-of-flight systems are in Refs.~\cite{detector} and \cite{MRPC}, respectively.
The background study is performed with a inclusive Monte Carlo (IMC) sample simulated with {\sc geant4}~\cite{sim}, 
which includes all known open-charm decays, charmless decays and initial-state radiative decays to $J/\psi$ or $\psi(3686)$. The decay amplitude is described by {\sc evtgen}~\cite{EvtGen}.
The tag and signal efficiency is determined by exclusive MC with $\psi(3770) \to D^{0} \bar{D}^{0}$, 
$D^{0} \to \pi^{-}\pi^{+}\eta$ and $\bar{D}^{0}$ decaying to four tag channels, which are 
$\bar{D}^{0} \to K^{+} \pi^{-}$, $\bar{D}^{0} \to K^{+} \pi^{-} \pi^{0}$, $\bar{D}^{0} \to K^{+} \pi^{-} \pi^{0} \pi^{0}$ 
and $\bar{D}^{0} \to K^{+} \pi^{-} \pi^{-} \pi^{+}$.
For the tag modes with more than two final particles, the decay models are from the amplitude fits to data~\cite{CLEO:2000fvk,BESIII:2019lwn,BESIII:2017jyh}.
For the signal channel, MC samples are firstly uniformed generated (PHSP) and then are generated with the amplitude model obtained from the fit to data (SIGNAL).
Here, through out this Letter, the charge conjugate, $\eta \to \gamma \gamma$ and $a_{0}(980) \to \pi \eta$ are implied 
Letter unless explicit point out.

For the data sample, a sample tagged by the four tag channels is selected with cut criteria on track reconstruction, particle identification and $\pi^{0}$ reconstruction being the same with Ref.~\cite{BESIII:2019xhl}, as well as the beam constraint mass ($M_{BC}$) and energy difference ($\Delta E$) windows are determined by five times of related resolutions, called as ``ST''. Within the ST, we search for the signal of $D^{0} \to \pi^{-} \pi^{+} \eta$, therefore the branching fraction 
of $D^{0} \to \pi^{-} \pi^{+} \eta$ is the fraction of the sample with signal relate to the whole tagged sample after efficiency corrections~\cite{MARK-III:1985hbd}.
Here for events with multiple candidates, the candidate with $\Delta E$ most close to 0 $GeV$ is selected. 
So the effect on background shape from this candidate selection is checked using IMC, from which it is found to be safe enough within at least $10.8\times$ data statistic.
For the sub-sample containing signal channel (called as ``DT''), a multi-variant analysis~\cite{Hocker:2007ht} is performed to suppress background from fake $\eta$. For variables, the invariant mass of $\gamma \gamma$, energy of the soft photon decaying from $\eta$, the $\chi^{2}$ of the fit with constraint the invariant mass of $\gamma \gamma$ to $\eta$ mass, and the helicity angle of the hard photon decaying from $\eta$ are trained with Gradient Boost Decision Tree according to the background and signal template given by IMC and PHSP samples. 
Here some cross-checks are performed and validate the data and MC being well consistent.
After MVA selection, the DT is further required a $K_{S}^{0}$ veto and a $M_{BC}$ mass window to suppress the peaking background $D^{0} \to K_{S}^{0} \eta$. 

The ST yields for each tag modes are determined by the fit to $M_{BC}$ of each ST sample; the DT yield is determined by the 
fit to $\Delta E$ of signal channel of DT sample. The detail fit plots are shown in Fig.~\ref{fig:tagY}. Here, the efficiency will be determined by SIGNAL MC sample.
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.20\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mbc_mode0.eps}
\put(-30,35){(a)}
\end{minipage}
\begin{minipage}[b]{0.20\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mbc_mode1.eps}
\put(-30,35){(b)}
\end{minipage}
\begin{minipage}[b]{0.20\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mbc_mode2.eps}
\put(-30,35){(c)}
\end{minipage}
\begin{minipage}[b]{0.20\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mbc_mode3.eps}
\put(-30,35){(d)}
\end{minipage}
\begin{minipage}[b]{0.40\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/D0_deltaE_withqqbar.eps}
\put(-50,75){(e)}
\end{minipage}
\caption{The plots of fit to the $M_{BC}$ of (a) $D^{0} \to K^{-}\pi^{+}$, (b) $D^{0} \to K^{-}\pi^{+} \pi^{0}$, 
(c) $D^{0} \to K^{-}\pi^{+} \pi^{0} \pi^{0}$ and (d) $D^{0} \to K^{-}\pi^{+} \pi^{+} \pi^{-}$. 
The blue lines are the total fits. The red dashed lines are the signal, parameterized with simulated shape. For (a,c), the simulated shape further convoluted 
with a Gaussian function to replace the small difference between data and MC.
The green dashed lines are the background, parameterized with Angus function.
The plot of fit to $\Delta E$ is shown in figure (e), where the background is parameterized as a 2$^{nd}$-order ChebyChev polynomial, the signal is parameterized with SIGNAL MC shape convoluted with a Gaussian function, the green and cyan histogram is the background estimated from IMC.}
\label{fig:tagY}
\end{center}
\end{figure}

To obtained the SIGNAL MC sample, the DT sample is divided into signal region ($|\Delta E|<0.45$~GeV) and side-band ($0.05<|\Delta E|<0.10$~GeV) according to Fig.~\ref{fig:tagY} (e),
then an full amplitude analysis is performed to analysis the $D^{0} \to \pi^{-}\pi^{+}\eta$ signal falling into the signal region, where the background shape is extracted from the data side-band. 
Therefore, we obtained a data sample of about 450 signal candidates with purity of $(70.7\pm2.1)$\% for amplitude analysis. 

The amplitude construction is almost the same with Ref.~\cite{BESIII:2019jjr} except for the shape of $\rho^{0}$, where both the $GS$ formalism~\cite{GS} and the $\rho^{0}-\omega$ mixing effect is considered as in Ref.~\cite{BESIII:2019ymv}.
In the amplitude fit, the largest orbital angular momentum hypothesis 2 due to the limit of decay phase of $D^{0}$. The magnitude and phase of $D^{0} \to \rho^{0}\eta$, obviously seen in the projection of $m(\pi^{-}\pi^{+})$,  is fixed to 1.0 and 0.0 and floated the magnitudes and phases of other intermediate processes.
Due to the large statistic fluctuation in data, all the amplitudes with significance 
than 3$\sigma$ will be considered. 
Further combine the fit quality, interference and correlations between the amplitudes, we finally retain four amplitudes to construct the fit model, which are $D^{0} \to \rho^{0} \eta$, $D^{0} \to a_{0}(980)^{-}\pi^{+}$, $D^{0} \to a_{0}(980)^{+}\pi^{-}$ and $D^{0} \to (\pi^{+}\eta)_{\mathrm{D-wave}}\pi^{-}$. 
Here we also check the significance of each amplitude and the $\rho^{0}-\omega$ mixing, 
as well as the the ratio $r_{+/-}$ with respect to the case in $D_{s}^{+} \to a_{0}(980)\pi$ decays (the case of theoretical prediction).
The projections on $m(\pi^{+}\eta)$, 
$m(\pi^{-}\eta)$ and $m(\pi^{-}\pi^{+})$, as well as the Dalitz plot of $m^{2}(\pi^{-}\eta)$ vs. $m^{2}(\pi^{+}\eta)$ for data (with background removed by sPlot method~\cite{Pivk:2004ty} through the fit shown in Fig.~\ref{fig:tagY} (e)) and SINGAL MC are shown in Fig.~\ref{fig:res}. 
\begin{figure}[htbp]
\begin{center}
\begin{minipage}[b]{0.15\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mpipeta.eps}
\put(-60,35){(a)}
\end{minipage}
\begin{minipage}[b]{0.15\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mpimeta.eps}
\put(-60,35){(b)}
\end{minipage}
\begin{minipage}[b]{0.15\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/mpipi.eps}
\put(-60,35){(c)}
\end{minipage}
\begin{minipage}[b]{0.23\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/histo_2D.eps}
\put(-60,65){(d)}
\end{minipage}
\begin{minipage}[b]{0.23\textwidth}
\epsfig{width=0.98\textwidth,clip=true,file=./figs/histo_2D_sigMC.eps}
\put(-50,65){(e)}
\end{minipage}
\caption{The projections on (a) $m(\pi^{+}\eta)$, (b) $m(\pi^{-}\eta)$ and (c) $m(\pi^{-}\pi^{+})$ as well as the Dalitz plots for (d) data (with background removed by sPlot method)
and (e) SIGNAL MC are shown. In figures (a-c), the blue lines are the fit curve, the green histograms are the background shapes and the dots with errors are the data.}
\label{fig:res}
\end{center}
\end{figure}

For the amplitude analysis, the systematic uncertainty are estimated from these sources:
1)
%The phase and fit fractions of the four amplitudes are listed in Tab.~\ref{tab:res}.
%\begin{table}[htbp]
%tiny
%\caption{The phases, fit fractions and statistical significance for each amplitude are listed. The uncertainties are statistical only.}
%\resizebox{\textwidth}{!}{% 
%\begin{tabular}{c|ccc} \hline
%Amplitude                                 & Phase            & Fit fraction (\%) & Significance ($\sigma$)       \\ \hline
%$D^{0} \to \rho^{0}\eta$                  & $0.00$ (fixed)   & $21.4\pm5.5$      & 5.4       \\
%$\rho - \omega$ mixing effect             & $2.21\pm0.18$    & $9.4\pm4.0$       & 3.1       \\
%$D^{0} \to a_{0}^{-}\pi^{+}$              & $0.74\pm0.34$    & $8.7\pm3.5$       & 3.9       \\
%$D^{0} \to a_{0}^{+}\pi^{-}$              &$-0.81\pm0.21$    & $50.8\pm7.4$      & 6.9       \\
%$D^{0} \to (\pi^{+}\eta)_{D-wave}\pi^{-}$ &$-0.02\pm0.25$    & $17.8\pm6.1$      & 3.9       \\	
%$r_{+/-}$                                 & -                & $5.9\pm2.2$       & 3.6 (5.7) \\
%\hline
%\end{tabular}
%%}
%\label{tab:res}
%\end{table}
%We also measure the branching fractions of $D^{0} \to \pi^{+} \pi^{-} \eta$ and $D^{0} \to \rho^{0} \eta$ with the amplitude model obtained from the data. 
%Especially for $\mathcal{B}(D^{0} \to \rho^{0} \eta)$, there is no experimental measurement but only predicted being varies of results 
%in theoretical interpretations for $D \to VP$ decay modes~\cite{Buccella:1994nf,Cheng:2010ry,Fu-Sheng:2011fji,Qin:2013tje,Jiang:2017zwr,Cheng:2019ggx}, which are listed in Tab.~\ref{tab:rhoetaph}.
%In the reference~\cite{Qin:2013tje}, the model FAT[mix] means that compared with the prediction given with FAT model, authors further consider the $\rho - \omega$ mixing effect to make the prediction match data better. Compared with the determination of the factorized parameters in the references~\cite{Qin:2013tje,Jiang:2017zwr}, the authors of reference~\cite{Cheng:2019ggx} extract the magnitude and strong phase of the topological amplitudes and predict the branching fraction of $D^{0} \to \rho^{0} \eta$ accordingly.
%\begin{table}[htbp]
%\begin{center}
%\caption{The branching fractions of $D^{0} \to \rho^{0} \eta$ for different theoretical interpretations with unit of $10^{-3}$.}
%\begin{tabular}{c|c} \hline
%Models                            & Theoretical predictions       \\ \hline
%FSI~\cite{Buccella:1994nf}        & $0.24$                        \\
%diagrammatic~\cite{Cheng:2010ry}  & $1.11\pm0.86$                 \\
%pole~\cite{Fu-Sheng:2011fji}      & $0.05\pm0.01$                 \\
%FAT~\cite{Qin:2013tje}            & $0.54$                        \\
%FAT[mix]~\cite{Qin:2013tje}       & $0.45$                        \\
%FAT~\cite{Jiang:2017zwr}	      & $1.4\pm0.2$                   \\
%Topological amplitudes~\cite{Cheng:2019ggx} & $0.31\pm0.05$ (for solution S3 in given reference) \\
%Topological amplitudes~\cite{Cheng:2019ggx} & $0.84\pm0.10$ (for solution S6 in given reference) \\
%\hline
%\end{tabular}
%\label{tab:rhoetaph}
%\end{center}
%\end{table}

%These experimental results on $D^{0} \to a_{0}^{\pm}\pi^{\mp}$ disagree with the theoretical prediction based on topological %amplitude~\cite{Cheng:2022vbw}: the branching fraction of $D^{0} \rightarrow a_{0}(980)^{+}\pi^{-}
%$D^{0} \rightarrow a_{0}(980)^{+}\pi^{-}~(a_{0}(980)^{-}\pi^{+})$ (In this theoretical interpretation, $a_{0}(980)^{\pm} \to K_{S}^{0}K^{\pm}$) being $1.3 \times 10^{-5}$ ($2.9\times 10^{-4}$).
